HunFlair2 in a cross-corpus evaluation of biomedical named entity recognition and normalization tools

With the exponential growth of the life science literature, biomedical text mining (BTM) has become an essential technology for accelerating the extraction of insights from publications. Identifying named entities (e.g., diseases, drugs, or genes) in texts and their linkage to reference knowledge bases are crucial steps in BTM pipelines to enable information aggregation from different documents. However, tools for these two steps are rarely applied in the same context in which they were developed. Instead, they are applied in the wild, i.e., on application-dependent text collections different from those used for the tools' training, varying, e.g., in focus, genre, style, and text type. This raises the question of whether the reported performance of BTM tools can be trusted for downstream applications. Here, we report on the results of a carefully designed cross-corpus benchmark for named entity extraction, where tools were applied systematically to corpora not used during their training. Based on a survey of 28 published systems, we selected five for an in-depth analysis on three publicly available corpora encompassing four different entity types. Comparison between tools results in a mixed picture and shows that, in a cross-corpus setting, the performance is significantly lower than the one reported in an in-corpus setting. HunFlair2 showed the best performance on average, being closely followed by PubTator. Our results indicate that users of BTM tools should expect diminishing performances when applying them in the wild compared to original publications and show that further research is necessary to make BTM tools more robust.

==> tables/comparison_hunflair_versions.tex <==
% Table generated by Excel2LaTeX from sheet 'Comparison HunFlairs'
\begin{table}[htbp]
  \centering
  \caption{Comparing F1-scores for NER in HunFlair versions 1 and 2.}
  \resizebox{\columnwidth}{!}{
    \begin{tabular}{lrrr}
\midrule    \textbf{Entity type / dataset} & \multicolumn{1}{l}{\textbf{HunFlair2}} & \multicolumn{1}{l}{\textbf{HunFlair-v1}} & \multicolumn{1}{l}{\textbf{Difference}} \\
    \midrule
    \textit{Chemical} &       &       &  \\
    BioID & 60.66 & 61.72 & \textit{-1.06} \\
    BioNLP2013 CG & 82.04 & 79.60 & \textit{+2.44} \\
    CRAFT & 58.99 & 58.41 & \textit{+0.58} \\
    MedMentions CTD & 58.73 & 53.76 & \textit{+4.97} \\
    \midrule
    \textit{Disease} &       &       &  \\
    BioNLP2013 CG & 56.66 & 60.73 & \textit{-4.07} \\
    CRAFT & 52.45 & 57.05 & \textit{-4.60} \\
    MedMentions CTD & 60.25 & 61.71 & \textit{-1.46} \\
    PDR   & 74.56 & 76.36 & \textit{-1.80} \\
    \midrule
    \textit{Gene} &       &       &  \\
    BioID & 62.09 & 63.74 & \textit{-1.65} \\
    BioNLP2013 CG & 86.90 & 83.44 & \textit{+3.46} \\
    CRAFT & 69.07 & 67.38 & \textit{+1.69} \\
    tmVar (v3) & 87.79 & 83.21 & \textit{+4.58} \\
    \midrule
    \textit{Species} &       &       &  \\
    BioID & 58.66 & 57.62 & \textit{+1.04} \\
    BioNLP2013 CG & 80.51 & 70.65 & \textit{+9.86} \\
    CRAFT & 86.92 & 84.86 & \textit{+2.06} \\
    \midrule
    Avg. Chemical & 65.10 & 63.38 & \textit{+1.72} \\
    Avg. Disease & 60.98 & 63.96 & \textit{-2.98} \\
    Avg. Gene & 76.46 & 74.44 & \textit{+2.02} \\
    Avg. Species & 75.36 & 71.04 & \textit{+4.32} \\
    \midrule
    Avg. All & 69.09 & 68.02 & \textit{+1.07} \\
    \bottomrule
    \end{tabular}%
    }
\label{tab:comparison_hunflair_versions}%
\end{table}%


==> tables/comparison_selected_tools.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
% \usepackage{lscape}
\afterpage{%
\begin{landscape}
\begin{table}[]
\caption{Comparison of selected tools}
\label{tab:comparison_tools}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
 &
  \multicolumn{2}{c}{\textbf{PubTator}} &
  \multicolumn{2}{c}{\textbf{BERN2}} &
  \multicolumn{2}{c}{\textbf{HunFlair2}} &
  \multicolumn{2}{c}{\textbf{SciSpacy}} &
  \multicolumn{2}{c}{\textbf{bent}} \\ \midrule
Entity type &
  NER &
  NEN &
  NER &
  NEN &
  NER &
  NEN &
  NER &
  NEN &
  NER &
  NEN \\ \midrule
\begin{tabular}[c]{@{}l@{}}  \\   \\   \\ Chemicals\end{tabular} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformers   \\ (GNormPlus,\\ BlueBERT-base)\\ $\sim$100 M parameters\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rule-based\\ (GNormPlus),\\ Statistical Inference\\ Network \end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Transformers\\ (RoBERTa),\\ $\sim$365 M parameters,\\ multi-task learning\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Rule-based\\ If no match: Transformers\\ (BioSyn SapBERT), \\ $\sim$100 M parameters\end{tabular}} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Transformers \\ BioLink-BERT-base), \\ $\sim$100 M parameters,\\ multi-task learning\end{tabular}} &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformers\\ (BioSyn SapBERT), \\ $\sim$100 M parameters\end{tabular}} &
  \multirow{5}{*}{Stack LSTMs} &
  \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Rule-based,\\ String matching\\ based on\\ character 3-grams\end{tabular}} &
  \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Transformers \\ (PubMed-BERT),\\ $\sim$100 M parameters\\ + Rule-based\\ post-processing\end{tabular}} &
  \multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}Rule-based \\ (Graph-based\\ approach)\end{tabular}} \\
\begin{tabular}[c]{@{}l@{}}  \\   \\   \\ Genes\end{tabular} &
   &
   &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(lr){2-3} \cmidrule(lr){5-5} \cmidrule(lr){7-7}
Species &
  \multicolumn{2}{c}{Rule-based (SR4GN)} &
   &
  \multirow{2}{*}{Rule-based only} &
   &
  \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Transformers\\ (SapBERT), \\ $\sim$100 M parameters\end{tabular}} &
   &
   &
   &
   \\ \cmidrule(lr){2-3}
\begin{tabular}[c]{@{}l@{}}  \\ Cell Lines\end{tabular} &
  \multicolumn{2}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Semi-Markov Models (TaggerOne),\\ joint extraction of NER and NEN\end{tabular}}} &
   &
   &
   &
   &
   &
   &
   &
   \\ \cmidrule(lr){5-5} \cmidrule(lr){7-7}
Diseases &
  \multicolumn{2}{c}{} &
   &
  \textit{see Chemicals and Genes} &
   &
  \textit{see Chemicals and Genes} &
   &
   &
   &
   \\ \cmidrule(lr){2-9}
Variants &
  CRF (tmVar 3.0) &
  Rule-based (tmVar 3.0) &
  CRF (tmVar 2.0) &
  Rule-based (tmVar 2.0) &
  \multicolumn{2}{c}{\textit{entity type not supported}} &
  \multicolumn{2}{c}{\textit{entity type not supported}} &
   &
   \\ \bottomrule
\end{tabular}%
}
\end{table}
\end{landscape}
}

==> tables/in_vs_cross_corpus.tex <==


% Table generated by Excel2LaTeX from sheet 'In-corpus'
\begin{table}[t!]
	\centering
	\caption{In-corpus results reported by PubTator~\cite{weiPubTatorCentralAutomated2019} and BERN2~\cite{Bern2AnAdvanMujeen} for named entity recognition (NER) and normalization (NEN).
		%
		For each tool and entity type we also provide the used evaluation corpus in parenthesis.
		%
		Note that, since the tools leverage different corpora for evaluation the results are not directly comparable, but they indicate the magnitude of the in-corpus test results.
		%
		Note also that the normalization results exclusively examine the NEN components and not (as in our study) in an end-to-end fashion NER and NEN combined.
		%
		We cannot report results for SciSpacy because they do not provide entity type-specific results.}
	\begin{tabular}{rrcc}
		\toprule
		\textbf{Task}                  &
		\textbf{Entity Type}           &
		\textbf{BERN2}                 &
		\textbf{PubTator}
		\\
		\midrule
		\multicolumn{1}{l}{NER}        &
		\multicolumn{1}{l}{  Chemical} &
		92.80                          &
		75.70
		\\
		                               &
		                               &
		\textit{(BC4CHEMD)}            &
		\textit{(NLM-Chem)}
		\\
		                               &
		\multicolumn{1}{l}{  Disease}  &
		88.60                          &
		82.90
		\\
		                               &
		                               &
		\textit{(NCBI-Disease)}        &
		\textit{(NCBI-Disease)}
		\\
		                               &
		\multicolumn{1}{l}{  Gene}     &
		83.70                          &
		88.10
		\\
		                               &
		                               &
		\textit{(BC2GM)}               &
		\textit{(NLM-Gene)}
		\\
		                               &
		\multicolumn{1}{l}{  Species}  &
		92.70                          &
		86.00
		\\
		                               &
		                               &
		\textit{(Linnaeus)}            &
		\textit{(Linnaeus)}
		\\
		\midrule
		\multicolumn{1}{l}{NEN}        &
		\multicolumn{1}{l}{  Chemical} &
		96.60                          &
		77.20
		\\
		                               &
		                               &
		\textit{(BC5CDR)}              &
		\textit{(NLM-Chem)}
		\\
		                               &
		\multicolumn{1}{l}{  Disease}  &
		93.90                          &
		80.70
		\\
		                               &
		                               &
		\textit{(BC5CDR)}              &
		\textit{(NCBI-Disease)}
		\\
		                               &
		\multicolumn{1}{l}{  Gene}     &
		95.90                          &
		85.90
		\\
		                               &
		                               &
		\textit{(BC2GM)}               &
		\textit{(NLM-Gene)}
		\\
		\bottomrule
	\end{tabular}%
	\label{tab:in_corpus_results}%
\end{table}%

% Table generated by Excel2LaTeX from sheet 'Tabelle1'
%\begin{table*}[htbp]
%  \centering
%  \caption{In-corpus results reported by PubTator and BERN2 for named entity recognition and normalization. We cannot report results for SciSpacy because they report results on the full corpora and not separately for each entity type.}
% Table generated by Excel2LaTeX from sheet 'Tabelle2'
%   \begin{tabular}{l|cccc|cccc}
%          & \multicolumn{4}{c|}{\textbf{NER}} & \multicolumn{4}{c}{\textbf{NEN}} \\
%    \textbf{Tool} & \textbf{Chemical} & \textbf{Disease} & \textbf{Gene} & \textbf{Species} & \textbf{Chemical} & \textbf{Disease} & \textbf{Gene} & \textbf{Species} \\
%    \midrule
%    \textit{PubTator} &       &       &       &       &       &       &       &  \\
%     In-corpus F1 & 75.70 & 82.90 & 88.10 & 86.00 & 77.20 & 80.70 & 85.90 & - \\
%     Dataset & NLM-Chem & NCBI-Disease & NLM-Gene & Linnaeus & NLM-Chem & NCBI-Disease & NLM-Gene & - \\
%    \midrule
%    \textit{Bern} &       &       &       &       &       &       &       &  \\
%     In-corpus F1 & 92.80 & 88.60 & 83.70 & 92.70 & 96.60 & 93.90 & 95.90 & - \\
%     Dataset & BC4CHEMD & NCBI-Disease & BC2GM & Linnaeus & BC5CDR & BC5CDR & BC2GN & - \\
%    \bottomrule
%    \end{tabular}%
%  \label{tab:in_corpus_results}%
%\end{table*}%


==> tables/medmentions_datasets.tex <==
% Table generated by Excel2LaTeX from sheet 'MedMentions'
\begin{table*}[htbp]
  \centering
  \caption{Difference between MedMentions to MetaMap SemGroups and MedMentions mapped to CTD}
    \begin{tabular}{lrrrrrrr}
    \toprule
    \textbf{Entity type / dataset} & \multicolumn{1}{l}{\textbf{HunFlair2}} & \multicolumn{1}{l}{\textbf{HunFlair-v1}} & \multicolumn{1}{l}{\textbf{BERN2}} & \multicolumn{1}{l}{\textbf{PubTator}} & \multicolumn{1}{l}{\textbf{SciSpacy}} & \multicolumn{1}{l}{\textbf{bent}} & \multicolumn{1}{l}{\textbf{Support}} \\
    \midrule
    \textit{Chemical} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  \\
    MedMentions SemGroups & 45.73 & 39.34 & 37.81 & 28.77 & 33.27 & 39.14 &           37,381  \\
    MedMentions CTD & 58.73 & 53.76 & 51.76 & 39.26 & 44.83 & 53.17 &           18,540  \\
    \midrule
    \textit{Disease} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  \\
    MedMentions SemGroups & 13.38 & 12.83 & 10.34 & 10.39 & 11.38 & 11.89 &           18,057  \\
    MedMentions CTD & 60.25 & 61.71 & 59.19 & 46.08 & 49.07 & 60.53 &           18,457  \\
    \bottomrule
    \end{tabular}%
  \label{tab:medmentions}%
\end{table*}%


==> tables/ner_results_20230904.tex <==
% Table generated by Excel2LaTeX from sheet 'NER-Results'
\begin{table*}[tbph]
  \centering
  \caption{NER results evaluated by F1 scores in a cross-corpus setting. The columns denote the examined tools and the rows denote the corpora split across the four entity types chemical, disease, gene and species. F1 scores in each row are represented by a color scale with the best value given in green and the worst value in red. Scores given in italics and colorless denote that the given tool was trained on the underlying corpus, i.e., does not give representative results in a cross-corpus setting. 
  $\dagger$ \anote{PubTator does not return any predictions for 4 documents}
  }
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Entity type / dataset} &
      \multicolumn{1}{c}{\textbf{BERN2}} &
      \multicolumn{1}{c}{\textbf{HunFlair2}} &
      \multicolumn{1}{c}{\textbf{PubTator}} &
      \multicolumn{1}{c}{\textbf{SciSpacy}} &
      \multicolumn{1}{c}{\textbf{bent}}
      \\
    \midrule
    \textit{Chemical} &
       &
       &
       &
       &
      
      \\
    \; BioID &
      \cellcolor[rgb]{ .996,  .839,  .408}59,15 &
      \cellcolor[rgb]{ .996,  .847,  .404}60,66 &
      \cellcolor[rgb]{ .969,  .733,  .486}40,09 &
      \cellcolor[rgb]{ .976,  .769,  .463}45,94 &
      \cellcolor[rgb]{ .996,  .843,  .408}59,67
      \\
    \; BioNLP2013 CG &
      \cellcolor[rgb]{ .796,  .835,  .494}77,96 &
      \cellcolor[rgb]{ .745,  .827,  .518}82,04 &
      \cellcolor[rgb]{ .996,  .847,  .404}60,47 &
      \cellcolor[rgb]{ .984,  .851,  .408}62,32 &
      \textit{84,08}
      \\
    \; CRAFT &
      \cellcolor[rgb]{ .996,  .835,  .412}58,57 &
      \cellcolor[rgb]{ .996,  .839,  .408}58,99 &
      \cellcolor[rgb]{ .957,  .702,  .51}33,77$\dagger$ &
      \cellcolor[rgb]{ .961,  .718,  .498}37,15 &
      \textit{75,16}
      \\
    \; MedMentions &
      \cellcolor[rgb]{ .984,  .796,  .443}50,81 &
      \cellcolor[rgb]{ .992,  .831,  .412}57,79 &
      \cellcolor[rgb]{ .965,  .725,  .49}38,53 &
      \cellcolor[rgb]{ .973,  .757,  .471}43,98 &
      \cellcolor[rgb]{ .984,  .804,  .435}52,20
      \\
    \midrule
    \textit{Disease} &
       &
       &
       &
       &
      
      \\
    \; BioNLP2013 CG &
      \cellcolor[rgb]{ .996,  .851,  .4}61,21 &
      \cellcolor[rgb]{ .992,  .827,  .42}56,66 &
      \cellcolor[rgb]{ .98,  .776,  .455}47,87 &
      \cellcolor[rgb]{ .984,  .796,  .439}51,28 &
      \cellcolor[rgb]{ .992,  .851,  .4}61,39
      \\
    \; CRAFT &
      \cellcolor[rgb]{ .988,  .808,  .431}52,99 &
      \cellcolor[rgb]{ .984,  .804,  .435}52,45 &
      \cellcolor[rgb]{ .957,  .694,  .514}32,27 $\dagger$&
      \cellcolor[rgb]{ .961,  .71,  .502}35,74 &
      \cellcolor[rgb]{ .984,  .804,  .435}52,62
      \\
    \; MedMentions &
      \cellcolor[rgb]{ .996,  .843,  .408}59,54 &
      \cellcolor[rgb]{ .992,  .851,  .404}61,44 &
      \cellcolor[rgb]{ .976,  .773,  .459}46,68 &
      \cellcolor[rgb]{ .98,  .788,  .447}49,87 &
      \cellcolor[rgb]{ .992,  .851,  .404}61,65
      \\
    \; PDR &
      \cellcolor[rgb]{ .859,  .839,  .467}72,80 &
      \cellcolor[rgb]{ .835,  .839,  .475}74,56 &
      \cellcolor[rgb]{ .945,  .847,  .424}65,45 &
      \cellcolor[rgb]{ .976,  .851,  .412}62,94 &
      \cellcolor[rgb]{ .82,  .835,  .482}75,77
      \\
    \midrule
    \textit{Gene} &
       &
       &
       &
       &
      
      \\
    \; BioID &
      \cellcolor[rgb]{ .992,  .851,  .4}61,42 &
      \cellcolor[rgb]{ .984,  .851,  .404}62,09 &
      \cellcolor[rgb]{ .973,  .851,  .412}63,07 &
      \cellcolor[rgb]{ .969,  .741,  .482}41,01 &
      \cellcolor[rgb]{ .988,  .851,  .404}61,85
      \\
    \; BioNLP2013 CG &
      \cellcolor[rgb]{ .792,  .831,  .498}78,35 &
      \cellcolor[rgb]{ .686,  .824,  .545}86,90 &
      \cellcolor[rgb]{ .827,  .835,  .478}75,21 &
      \cellcolor[rgb]{ .992,  .824,  .42}55,83 &
      \textit{87,01}
      \\
    \; CRAFT &
      \cellcolor[rgb]{ .988,  .812,  .431}53,80 &
      \cellcolor[rgb]{ .902,  .843,  .443}69,07 &
      \cellcolor[rgb]{ .835,  .839,  .475}74,60 $\dagger$&
      \cellcolor[rgb]{ .98,  .788,  .447}49,83 &
      \textit{79,95}
      \\
    \; tmVar (v3) &
      \cellcolor[rgb]{ .98,  .78,  .451}48,05 &
      \cellcolor[rgb]{ .678,  .824,  .549}87,79 &
      \cellcolor[rgb]{ .663,  .82,  .557}88,82 &
      \cellcolor[rgb]{ .949,  .847,  .424}65,26 &
      \cellcolor[rgb]{ .745,  .827,  .518}82,27
      \\
    \midrule
    \textit{Species} &
       &
       &
       &
       &
      
      \\
    \; BioID &
      \cellcolor[rgb]{ 1,  .851,  .4}60,80 &
      \cellcolor[rgb]{ .996,  .839,  .412}58,66 &
      \cellcolor[rgb]{ .996,  .847,  .404}60,35 &
      \cellcolor[rgb]{ .973,  .757,  .471}43,94 &
      \cellcolor[rgb]{ .953,  .847,  .42}64,91
      \\
    \; BioNLP2013 CG &
      \cellcolor[rgb]{ .753,  .831,  .514}81,31 &
      \cellcolor[rgb]{ .765,  .831,  .51}80,51 &
      \cellcolor[rgb]{ .737,  .827,  .522}82,68 &
      \cellcolor[rgb]{ .973,  .761,  .467}44,89 &
      \textit{92,43}
      \\
    \; CRAFT &
      \cellcolor[rgb]{ .682,  .824,  .545}87,24 &
      \cellcolor[rgb]{ .686,  .824,  .545}86,92 &
      \cellcolor[rgb]{ .761,  .831,  .51}80,79 &
      \cellcolor[rgb]{ .961,  .714,  .502}36,04 &
      \textit{95,94}
      \\
    \midrule
    Avg. Chemical &
      \cellcolor[rgb]{ .992,  .851,  .404}61,62 &
      \cellcolor[rgb]{ .953,  .847,  .42}64,87 &
      \cellcolor[rgb]{ .973,  .753,  .471}43,21 &
      \cellcolor[rgb]{ .976,  .776,  .455}47,35 &
      \textit{67,78}
      \\
    Avg. Disease &
      \cellcolor[rgb]{ .992,  .851,  .404}61,64 &
      \cellcolor[rgb]{ .996,  .851,  .4}61,28 &
      \cellcolor[rgb]{ .98,  .78,  .451}48,07 &
      \cellcolor[rgb]{ .98,  .788,  .443}49,96 &
      \cellcolor[rgb]{ .976,  .851,  .412}62,86
      \\
    Avg. Gene &
      \cellcolor[rgb]{ .996,  .847,  .404}60,41 &
      \cellcolor[rgb]{ .812,  .835,  .486}76,46 &
      \cellcolor[rgb]{ .827,  .835,  .478}75,42 &
      \cellcolor[rgb]{ .988,  .808,  .431}52,98 &
      \textit{77,77}
      \\
    Avg. Species &
      \cellcolor[rgb]{ .812,  .835,  .486}76,45 &
      \cellcolor[rgb]{ .827,  .835,  .478}75,36 &
      \cellcolor[rgb]{ .835,  .839,  .475}74,61 &
      \cellcolor[rgb]{ .969,  .745,  .478}41,62 &
      \textit{84,43}
      \\
    \midrule
    Avg. All &
      \cellcolor[rgb]{ .961,  .847,  .42}64,27 &
      \cellcolor[rgb]{ .902,  .843,  .443}69,10 &
      \cellcolor[rgb]{ .996,  .843,  .408}59,38 &
      \cellcolor[rgb]{ .98,  .78,  .451}48,40 &
      \textit{72,46}
      \\
    \bottomrule
    \end{tabular}%
    \label{tab:ner_results}%
\end{table*}%


==> tables/ner_results_20230906.tex <==
% Table generated by Excel2LaTeX from sheet 'NER-Results'
\begin{table*}[tbhp]
  \centering
  \caption{NER results evaluated by F1 scores in a cross-corpus setting. The columns denote the examined tools and the rows denote the corpora split across the four entity types chemical, disease, gene and species. F1 scores in each row are represented by a color scale with the best value given in green and the worst value in red. Scores given in italics and colorless denote that the given tool was trained on the underlying corpus, i.e., does not give representative results in a cross-corpus setting. 
  $\dagger$ \anote{PubTator does not return any predictions for 4 documents}
  }
    \begin{tabular}{lrrrrr}
    \toprule
    \textbf{Entity type / dataset} &
      \multicolumn{1}{c}{\textbf{BERN2}} &
      \multicolumn{1}{c}{\textbf{HunFlair2}} &
      \multicolumn{1}{c}{\textbf{PubTator}} &
      \multicolumn{1}{c}{\textbf{SciSpacy}} &
      \multicolumn{1}{c}{\textbf{bent}}
      \\
    \midrule
    \textit{Chemical} &
       &
       &
       &
       &
      
      \\
    BioID &
      \cellcolor[rgb]{ 1,  .851,  .4}59.15 &
      \cellcolor[rgb]{ .663,  .82,  .557}60.66 &
      \cellcolor[rgb]{ .957,  .694,  .514}40.09 &
      \cellcolor[rgb]{ .969,  .741,  .482}45.94 &
      \cellcolor[rgb]{ .886,  .843,  .451}59.67
      \\
    BioNLP2013 CG &
      \cellcolor[rgb]{ .78,  .831,  .502}77.96 &
      \cellcolor[rgb]{ .663,  .82,  .557}82.04 &
      \cellcolor[rgb]{ .957,  .694,  .514}60.47 &
      \cellcolor[rgb]{ .965,  .722,  .494}62.32 &
      \textit{84.08}
      \\
    CRAFT &
      \cellcolor[rgb]{ .678,  .824,  .549}58.57 &
      \cellcolor[rgb]{ .663,  .82,  .557}58.99 &
      \cellcolor[rgb]{ .957,  .694,  .514}33.77 &
      \cellcolor[rgb]{ .965,  .729,  .49}37.15 &
      \textit{75.16}
      \\
    MedMentions &
      \cellcolor[rgb]{ 1,  .851,  .4}50.81 &
      \cellcolor[rgb]{ .663,  .82,  .557}57.79 &
      \cellcolor[rgb]{ .957,  .694,  .514}38.53 &
      \cellcolor[rgb]{ .973,  .761,  .467}43.98 &
      \cellcolor[rgb]{ .933,  .847,  .427}52.20
      \\
    \midrule
    \textit{Disease} &
       &
       &
       &
       &
      
      \\
    BioNLP2013 CG &
      \cellcolor[rgb]{ .678,  .824,  .549}61.21 &
      \cellcolor[rgb]{ 1,  .851,  .4}56.66 &
      \cellcolor[rgb]{ .957,  .694,  .514}47.87 &
      \cellcolor[rgb]{ .973,  .753,  .471}51.28 &
      \cellcolor[rgb]{ .663,  .82,  .557}61.39
      \\
    CRAFT &
      \cellcolor[rgb]{ .663,  .82,  .557}52.99 &
      \cellcolor[rgb]{ 1,  .851,  .4}52.45 &
      \cellcolor[rgb]{ .957,  .694,  .514}32.27 &
      \cellcolor[rgb]{ .961,  .718,  .498}35.74 &
      \cellcolor[rgb]{ .894,  .843,  .447}52.62
      \\
    MedMentions &
      \cellcolor[rgb]{ 1,  .851,  .4}59.54 &
      \cellcolor[rgb]{ .698,  .824,  .541}61.44 &
      \cellcolor[rgb]{ .957,  .694,  .514}46.68 &
      \cellcolor[rgb]{ .965,  .729,  .486}49.87 &
      \cellcolor[rgb]{ .663,  .82,  .557}61.65
      \\
    PDR &
      \cellcolor[rgb]{ 1,  .851,  .4}72.80 &
      \cellcolor[rgb]{ .804,  .835,  .49}74.56 &
      \cellcolor[rgb]{ .965,  .733,  .486}65.45 &
      \cellcolor[rgb]{ .957,  .694,  .514}62.94 &
      \cellcolor[rgb]{ .663,  .82,  .557}75.77
      \\
    \midrule
    \textit{Gene} &
       &
       &
       &
       &
      
      \\
    BioID &
      \cellcolor[rgb]{ .996,  .847,  .404}61.42 &
      \cellcolor[rgb]{ .937,  .847,  .427}62.09 &
      \cellcolor[rgb]{ .663,  .82,  .557}63.07 &
      \cellcolor[rgb]{ .957,  .694,  .514}41.01 &
      \cellcolor[rgb]{ 1,  .851,  .4}61.85
      \\
    BioNLP2013 CG &
      \cellcolor[rgb]{ .949,  .847,  .424}78.35 &
      \cellcolor[rgb]{ .663,  .82,  .557}86.90 &
      \cellcolor[rgb]{ .996,  .839,  .412}75.21 &
      \cellcolor[rgb]{ .957,  .694,  .514}55.83 &
      \textit{87.01}
      \\
    CRAFT &
      \cellcolor[rgb]{ .969,  .745,  .478}53.80 &
      \cellcolor[rgb]{ .808,  .835,  .49}69.07 &
      \cellcolor[rgb]{ .663,  .82,  .557}74.60 &
      \cellcolor[rgb]{ .957,  .694,  .514}49.83 &
      \textit{79.95}
      \\
    tmVar (v3) &
      \cellcolor[rgb]{ .957,  .694,  .514}48.05 &
      \cellcolor[rgb]{ .718,  .827,  .529}87.79 &
      \cellcolor[rgb]{ .663,  .82,  .557}88.82 &
      \cellcolor[rgb]{ .976,  .773,  .459}65.26 &
      \cellcolor[rgb]{ 1,  .851,  .4}82.27
      \\
    \midrule
    \textit{Species} &
       &
       &
       &
       &
      
      \\
    BioID &
      \cellcolor[rgb]{ .969,  .851,  .412}60.80 &
      \cellcolor[rgb]{ .992,  .831,  .412}58.66 &
      \cellcolor[rgb]{ 1,  .851,  .4}60.35 &
      \cellcolor[rgb]{ .957,  .694,  .514}43.94 &
      \cellcolor[rgb]{ .663,  .82,  .557}64.91
      \\
    BioNLP2013 CG &
      \cellcolor[rgb]{ .925,  .847,  .435}81.31 &
      \cellcolor[rgb]{ .996,  .847,  .404}80.51 &
      \cellcolor[rgb]{ .663,  .82,  .557}82.68 &
      \cellcolor[rgb]{ .957,  .694,  .514}44.89 &
      \textit{92.43}
      \\
    CRAFT &
      \cellcolor[rgb]{ .663,  .82,  .557}87.24 &
      \cellcolor[rgb]{ .698,  .824,  .541}86.92 &
      \cellcolor[rgb]{ .996,  .839,  .408}80.79 &
      \cellcolor[rgb]{ .957,  .694,  .514}36.04 &
      \textit{95.94}
      \\
    \midrule
    Avg. Chemical &
      \cellcolor[rgb]{ .769,  .831,  .506}61.62 &
      \cellcolor[rgb]{ .663,  .82,  .557}64.87 &
      \cellcolor[rgb]{ .957,  .694,  .514}43.21 &
      \cellcolor[rgb]{ .973,  .749,  .475}47.35 &
      \textit{67.78}
      \\
    Avg. Disease &
      \cellcolor[rgb]{ .925,  .847,  .435}61.64 &
      \cellcolor[rgb]{ 1,  .851,  .4}61.28 &
      \cellcolor[rgb]{ .957,  .694,  .514}48.07 &
      \cellcolor[rgb]{ .961,  .714,  .498}49.96 &
      \cellcolor[rgb]{ .663,  .82,  .557}62.86
      \\
    Avg. Gene &
      \cellcolor[rgb]{ .976,  .769,  .459}60.41 &
      \cellcolor[rgb]{ .663,  .82,  .557}76.46 &
      \cellcolor[rgb]{ .706,  .824,  .537}75.42 &
      \cellcolor[rgb]{ .957,  .694,  .514}52.98 &
      \textit{77.77}
      \\
    Avg. Species &
      \cellcolor[rgb]{ .663,  .82,  .557}76.45 &
      \cellcolor[rgb]{ .914,  .843,  .439}75.36 &
      \cellcolor[rgb]{ .996,  .847,  .404}74.61 &
      \cellcolor[rgb]{ .957,  .694,  .514}41.62 &
      \textit{84.43}
      \\
    \midrule
    Avg. All &
      \cellcolor[rgb]{ .89,  .843,  .451}64.27 &
      \cellcolor[rgb]{ .663,  .82,  .557}69.10 &
      \cellcolor[rgb]{ .988,  .82,  .424}59.38 &
      \cellcolor[rgb]{ .957,  .694,  .514}48.40 &
      \textit{72.46}
      \\
    \bottomrule
    \end{tabular}%
  \label{tab:ner_results}%
\end{table*}%




==> tables/ner_results_lenient_20230904.tex <==
% Table generated by Excel2LaTeX from sheet 'NER-Results-lenient-table'
\begin{table*}[tbhp]
  \centering
  \caption{Named entity recognition results using a lenient evaluation setting, i.e. we count each prediction as true positive which is a sub- or superstring of gold standard entity mention.}
    \begin{tabular}{lcccccccc}
        \toprule
     &
      \multicolumn{2}{c}{\textbf{BERN2}} &
      \multicolumn{2}{c}{\textbf{HunFlair2}} &
      \multicolumn{2}{c}{\textbf{PubTator}} &
      \multicolumn{2}{c}{\textbf{SciSpacy}}
      \\
     &
      \textbf{Lenient F1} &
      \textbf{Difference} &
      \textbf{Lenient F1} &
      \textbf{Difference} &
      \textbf{Lenient F1} &
      \textbf{Difference} &
      \textbf{Lenient F1} &
      \textbf{Difference}
      \\
    \midrule
    Avg. Chemical &
      66.12 &
      \textit{+ 4.50} &
      69.44 &
      \textit{+ 4.57} &
      49.12 &
      \textit{+ 5.91} &
      52.14 &
      \textit{+ 4.79}
      \\
    Avg. Disease &
      72.35 &
      \textit{+ 10.71} &
      70.43 &
      \textit{+ 9.15} &
      61.06 &
      \textit{+ 12.99} &
      63.14 &
      \textit{+ 13.18}
      \\
    Avg. Gene &
      87.34 &
      \textit{+ 26.93} &
      87.10 &
      \textit{+ 10.64} &
      78.11 &
      \textit{+ 2.69} &
      64.90 &
      \textit{+ 11.92}
      \\
    Avg. Species &
      81.64 &
      \textit{+ 5.19} &
      81.55 &
      \textit{+ 6.19} &
      78.16 &
      \textit{+ 3.55} &
      59.47 &
      \textit{+ 17.85}
      \\
    \midrule
    Avg. All &
      76.54 &
      \textit{+ 12.27} &
      76.84 &
      \textit{+ 7.74} &
      65.84 &
      \textit{+ 6.46} &
      59.94 &
      \textit{+ 11.54}
      \\
      \bottomrule
    \end{tabular}%
  \label{tab:lenient_ner_results}%
\end{table*}%


==> tables/ner_results_mention_20231102.tex <==
% Table generated by Excel2LaTeX from sheet 'NEN-Mention-Level'
\begin{table*}[tbhp]
	\centering
	\caption{Mention-level cross-corpus $mu$F1 for named entity extraction, i.e. end-to-end entity recognition and normalization.
		% Colour-coding is applied per row and evaluation metric separately highlighting the best values in green and the worst in red.
		% $\dagger$ \anote{PubTator does not return any predictions for 4 documents}
		% See Section \nameref{sec:evaluation_nen}
	}
	% bern  hunflair-transformers-aio  pubtator  scispacy_ner_nen   bent
	% f1  41.12                      44.46      30.8             33.92  40.48
	\begin{tabular}{lrrrrrrrrrrr}
    \textbf{Unique Mentions} &       &       &       &       &       &       &       &       &       &       &  \\
          &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Entity type / dataset} & \multicolumn{1}{l}{\textbf{Support}} & \multicolumn{2}{c}{\textbf{BERN2}} & \multicolumn{2}{c}{\textbf{HunFlair2}} & \multicolumn{2}{c}{\textbf{PubTator}} & \multicolumn{2}{c}{\textbf{SciSpacy}} & \multicolumn{2}{c}{\textbf{bent}} \\
          &       & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} \\
    \midrule
    \textit{Chemical} &       &       &       &       &       &       &       &       &       &       &  \\
    MedMentions & 6450  & 32.56 & \textit{-18.25} & 37.31 & \textit{-20.48} & 21.82 & \textit{\textbf{-16.71}} & 24.49 & \textit{-19.49} & 34.52 & \textit{-17.68} \\
    \midrule
    \textit{Disease} &       &       &       &       &       &       &       &       &       &       &  \\
    MedMentions & 5449  & 31.16 & \textit{-28.38} & 32.40 & \textit{-29.04} & 20.30 & \textit{\textbf{-26.38}} & 22.38 & \textit{-27.49} & 32.19 & \textit{-29.46} \\
    \textit{Gene} &       &       &       &       &       &       &       &       &       &       &  \\
    tmVar (v3) & 1237  & 25.68 & \textit{-22.37} & 66.34 & \textit{-21.45} & 71.68 & \textit{\textbf{-17.14}} & 37.51 & \textit{-27.75} & 57.80 & \textit{-24.47} \\
    \midrule
    \textit{Species} &       &       &       &       &       &       &       &       &       &       &  \\
    BioID & 442   & 13.91 & \textit{-46.89} & 14.28 & \textit{-44.38} & 15.87 & \textit{-44.48} & 5.74  & \textit{\textbf{-38.20}} & 24.15 & \textit{-40.76} \\
    Avg. All & 13578 & 25.83 & \textit{-28.97} & 37.58 & \textit{-28.84} & 32.42 & \textit{\textbf{-26.18}} & 22.53 & \textit{-28.23} & 37.17 & \textit{-28.09} \\
    \midrule
          &       &       &       &       &       &       &       &       &       &       &  \\
    \textbf{Unique Mentions and Lenient} &       &       &       &       &       &       &       &       &       &       &  \\
          &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Entity type / dataset} & \multicolumn{1}{l}{\textbf{Support}} & \multicolumn{2}{c}{\textbf{BERN2}} & \multicolumn{2}{c}{\textbf{HunFlair2}} & \multicolumn{2}{c}{\textbf{PubTator}} & \multicolumn{2}{c}{\textbf{SciSpacy}} & \multicolumn{2}{c}{\textbf{bent}} \\
          &       & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} & \textbf{F1} & \textbf{Difference} \\
    \midrule
    \textit{Chemical} &       &       &       &       &       &       &       &       &       &       &  \\
    MedMentions & 6450  & 40.55 & \textit{-10.26} & 45.29 & \textit{-12.50} & 28.96 & \textit{\textbf{-9.57}} & 30.28 & \textit{-13.70} & 42.16 & \textit{-10.04} \\
    \midrule
    \textit{Disease} &       &       &       &       &       &       &       &       &       &       &  \\
    MedMentions & 5449  & 44.94 & \textit{-14.60} & 46.02 & \textit{-15.42} & 34.76 & \textit{\textbf{-11.92}} & 37.50 & \textit{-12.37} & 46.78 & \textit{-14.87} \\
    \textit{Gene} &       &       &       &       &       &       &       &       &       &       &  \\
    tmVar (v3) & 1237  & 77.07 & \textit{\textbf{29.02}} & 77.60 & \textit{-10.19} & 73.59 & \textit{-15.23} & 60.91 & \textit{-4.35} & 75.29 & \textit{-6.98} \\
    \midrule
    \textit{Species} &       &       &       &       &       &       &       &       &       &       &  \\
    BioID & 442   & 44.34 & \textit{-16.46} & 46.42 & \textit{\textbf{-12.24}} & 19.06 & \textit{-41.29} & 21.38 & \textit{-22.56} & 37.85 & \textit{-27.06} \\
    Avg. All & 13578 & 51.73 & \textit{\textbf{-3.08}} & 53.83 & \textit{-12.59} & 39.09 & \textit{-19.50} & 37.52 & \textit{-13.25} & 50.52 & \textit{-14.74} \\
    \bottomrule
    \end{tabular}%
	\label{tab:nen_results_ml}%
\end{table*}%


==> tables/results_macro_20230904.tex <==
% Table generated by Excel2LaTeX from sheet 'NER-Macro-F1-Combined'
\begin{table*}[tbhp]
	\centering
	\caption{Macro F1 scores over unique mentions. We report results for our standard (first row) and
		lenient evaluation setting (second row) and
		compare the results to the default micro-average F1 evaluation scores in Table \ref{tab:ner_results} and
		\ref{tab:lenient_ner_results} for each entity type.}
	\begin{tabular}{rrcccccccc}
		\toprule
		                                                         &
		\multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Support}}} &
		\multicolumn{2}{c}{\textbf{BERN2}}                       &
		\multicolumn{2}{c}{\textbf{HunFlair2}}                 &
		\multicolumn{2}{c}{\textbf{PubTator}}                    &
		\multicolumn{2}{c}{\textbf{SciSpacy}}
		\\
		                                                         &
		                                                         &
		\textbf{Macro F1}                                        &
		\textbf{Difference}                                      &
		\textbf{Macro F1}                                        &
		\textbf{Difference}                                      &
		\textbf{Macro F1}                                        &
		\textbf{Difference}                                      &
		\textbf{Macro F1}                                        &
		\textbf{Difference}
		\\
		\midrule
		\multicolumn{1}{l}{Chemical}                             &
		9748                                                     &
		40.36                                                    &
		\textit{-21.26}                                          &
		41.37                                                    &
		\textit{-23.50}                                          &
		22.18                                                    &
		\textit{-21.03}                                          &
		26.70                                                    &
		\textit{-20.65}
		\\
		                                                         &
		                                                         &
		49.26                                                    &
		\textit{-16.86}                                          &
		50.91                                                    &
		\textit{-19.52}                                          &
		30.27                                                    &
		\textit{-18.85}                                          &
		34.31                                                    &
		\textit{-17.83}
		\\
		\multicolumn{1}{l}{Disease}                              &
		7293                                                     &
		31.25                                                    &
		\textit{-30.39}                                          &
		31.33                                                    &
		\textit{-29.95}                                          &
		20.95                                                    &
		\textit{-27.12}                                          &
		22.66                                                    &
		\textit{-27.30}
		\\
		                                                         &
		                                                         &
		49.64                                                    &
		\textit{-22.71}                                          &
		47.42                                                    &
		\textit{-23.01}                                          &
		38.86                                                    &
		\textit{-22.20}                                          &
		40.92                                                    &
		\textit{-22.22}
		\\
		\multicolumn{1}{l}{Gene}                                 &
		10597                                                    &
		30.21                                                    &
		\textit{-30.20}                                          &
		51.57                                                    &
		\textit{-24.89}                                          &
		51.22                                                    &
		\textit{-24.20}                                          &
		27.30                                                    &
		\textit{-25.68}
		\\
		                                                         &
		                                                         &
		73.71                                                    &
		\textit{-13.63}                                          &
		72.36                                                    &
		\textit{-14.74}                                          &
		58.44                                                    &
		\textit{-19.67}                                          &
		52.10                                                    &
		\textit{-12.80}
		\\
		\multicolumn{1}{l}{Species}                              &
		1099                                                     &
		27.00                                                    &
		\textit{-49.45}                                          &
		26.34                                                    &
		\textit{-49.02}                                          &
		24.84                                                    &
		\textit{-49.77}                                          &
		5.61                                                     &
		\textit{-36.01}
		\\
		                                                         &
		                                                         &
		44.50                                                    &
		\textit{-37.14}                                          &
		45.89                                                    &
		\textit{-35.66}                                          &
		32.00                                                    &
		\textit{-46.16}                                          &
		37.22                                                    &
		\textit{-22.25}
		\\
		\midrule
		\multicolumn{1}{l}{All}                                  &
		28737                                                    &
		32.55                                                    &
		\textit{-31.72}                                          &
		38.41                                                    &
		\textit{-30.69}                                          &
		30.13                                                    &
		\textit{-29.25}                                          &
		21.56                                                    &
		\textit{-26.84}
		\\
		                                                         &
		                                                         &
		54.93                                                    &
		\textit{-21.61}                                          &
		54.69                                                    &
		\textit{-22.15}                                          &
		40.42                                                    &
		\textit{-25.42}                                          &
		41.40                                                    &
		\textit{-18.54}
		\\
		\bottomrule
	\end{tabular}%
	\label{tab:ner_results_entity_distribution}%
\end{table*}

\begin{table*}[tbhp]
	\centering
	\caption{Micro ($\mu$) and macro (M) F1 scores by entity type.
		Micro scores are computed with mentions individually, while macro are the average over per entity F1 scores.}
	\label{tab:nen_results_entity_distribution}              %

	\resizebox{\textwidth}{!}{
		\begin{tabular}{ll|ccc|ccc|ccc|ccc|ccc}
			\toprule
			            &          & \multicolumn{3}{r}{BERN2} & \multicolumn{3}{r}{HunFlair (v2)} & \multicolumn{3}{r}{PubTator} & \multicolumn{3}{r}{SciSpacy} & \multicolumn{3}{r}{bent}                                                                                              \\
			            &          & $\mu$ F1                  & M F1                              & Diff                         & $\mu$ F1                     & M F1                     & Diff   & $\mu$ F1 & M F1  & Diff   & $\mu$ F1 & M F1  & Diff   & $\mu$ F1 & M F1  & Diff   \\
			\midrule
			MedMentions & Chemical & 41.68                     & 28.20                             & -13.48                       & 45.16                        & 27.62                    & -17.54 & 31.26    & 20.19 & -11.07 & 34.94    & 29.58 & -5.36  & 40.97    & 26.10 & -14.87 \\
			MedMentions & Disease  & 47.31                     & 27.70                             & -19.61                       & 48.89                        & 28.07                    & -20.82 & 41.05    & 23.40 & -17.65 & 40.76    & 33.82 & -6.94  & 46.04    & 21.80 & -24.24 \\
			tmVar v3    & Gene     & 43.81                     & 24.85                             & -18.96                       & 75.71                        & 46.38                    & -29.33 & 85.92    & 71.41 & -14.51 & 0.00     & 0.00  & 0.00   & 0.54     & 0.29  & -0.25  \\
			BioID       & Species  & 14.35                     & 14.19                             & -0.16                        & 50.71                        & 7.05                     & -43.66 & 58.90    & 18.19 & -40.71 & 37.14    & 2.69  & -34.45 & 10.33    & 2.29  & -8.04  \\
			\bottomrule
		\end{tabular}
		% 	\toprule
		% 	         & \multicolumn{3}{c|}{\textbf{BERN2}}
		% 	         & \multicolumn{3}{c|}{\textbf{HunFlair2}}
		% 	         & \multicolumn{3}{c|}{\textbf{PubTator}}
		% 	         & \multicolumn{3}{c|}{\textbf{SciSpacy}}
		% 	         & \multicolumn{3}{c}{\textbf{bent}}
		% 	\\
		% 	         & \textbf{$\mu$ F1}                         & \textbf{M F1} & \textbf{Diff}
		% 	         & \textbf{$\mu$ F1}                         & \textbf{M F1} & \textbf{Diff}
		% 	         & \textbf{$\mu$ F1}                         & \textbf{M F1} & \textbf{Diff}
		% 	         & \textbf{$\mu$ F1}                         & \textbf{M F1} & \textbf{Diff}
		% 	         & \textbf{$\mu$ F1}                         & \textbf{M F1} & \textbf{Diff}                                                                                                     \\
		%
		% 	\midrule
		% 	Species  & 14.79                                     & 17.95         & +3.16         & 29.61 & 10.95 & -18.65 & 30.26 & 17.69 & -12.57 & 18.33 & 3.36  & -14.97 & -     & -     & -      \\
		% 	Disease  & 45.88                                     & 25.85         & -20.03        & 46.99 & 26.50 & -20.49 & 39.06 & 22.04 & -17.02 & 38.49 & 32.54 & -5.95  & 44.64 & 20.63 & -24.01 \\
		% 	Chemical & 33.42                                     & 22.48         & -10.94        & 45.16 & 27.62 & -17.53 & 31.26 & 20.19 & -11.07 & 34.94 & 29.58 & -5.37  & 40.97 & 26.10 & -14.86 \\
		% 	Gene     & 43.81                                     & 24.85         & -18.95        & 75.71 & 46.38 & -29.33 & 85.92 & 71.41 & -14.51 & -     & -     & -      & 0.54  & 0.29  & -0.25  \\
		% 	\bottomrule
		% \end{tabular}
	}
\end{table*}

